SpeechGPT: Empowering Large Language Models with Intrinsic Cross-Modal Conversational Abilities

Multi-modal large language models are regarded as a crucial step towards Artificial General Intelligence (AGI) and have garnered significant interest with the emergence of ChatGPT. However, current speech-language models typically adopt the cascade paradigm, preventing inter-modal knowledge transfer. In this paper, we propose SpeechGPT, a large language model with intrinsic cross-modal conversational abilities, capable of perceiving and generating multi-model content. With discrete speech representations, we first construct SpeechInstruct, a large-scale cross-modal speech instruction dataset. Additionally, we employ a three-stage training strategy that includes modality-adaptation pre-training, cross-modal instruction fine-tuning, and chain-of-modality instruction fine-tuning. The experimental results demonstrate that SpeechGPT has an impressive capacity to follow multi-modal human instructions and highlight the potential of handling multiple modalities with one model. Demos are shown in https://0nutation.github.io/SpeechGPT.github.io/.

==> Sections/010_introduction_v1.tex <==
Conversational large language models like ChatGPT have made significant strides in generating contextually relevant, coherent, and informative responses.
Despite the remarkable achievements, there is a growing demand for models that can effectively engage in spoken conversational interactions.



==> Sections/041_datasets.tex <==
\noindent\textbf{Further Pretraining}~


==> Tables/hyper_params.tex <==
\begin{table}[htb]
    % \setlength{\abovecaptionskip}{-0.cm}
    % \setlength{\belowcaptionskip}{-0.2cm}
    % \small
    \centering
    \begin{tabular}{lccc}
        \toprule
         & \textbf{Stage 1} 
         & \textbf{Stage 2}
         & \textbf{Stage 3}
         \\
        \midrule
        Batch size & 768 & 1536 & 128 \\
        Peak learning rate & 2e-4 & 2e-4 & 2e-4 \\
        Max length & 1024 & 512 & 1024 \\
        Training steps & 900 & 4000 & 4200 \\
        LoRA rank & - & - & 8\\
        LoRA alpha & - & - & 16\\
        Trainable parameters & 13B & 13B & 6M \\
        Training device & 96 $\times$ A100 & 96 $\times$ A100 & 8 $\times$ A100 \\
        \bottomrule
    \end{tabular}
    \captionsetup{skip=10pt}
    \caption{SpeechGPT training hyperparameters. 
    }
    \label{tab:hyper_params}
\end{table}
